Asymptotic Theory of Bayes Factor in Stochastic Differential Equations: Part I

Research on asymptotic model selection in the context of stochastic differential equations (SDEs) is almost non-existent in the literature. In particular, when a collection of SDEs is considered, the problem of asymptotic model selection has not been hitherto investigated. Indeed, even though the diffusion coefficients may be considered known, questions on appropriate choice of the drift functions constitute a non-trivial model selection problem. In this article, we develop the asymptotic theory for comparisons between collections of SDEs with respect to the choice of drift functions using Bayes factors when the number of equations (individuals) in the collection of SDEs tend to infinity while the time domains remain bounded for each equation. Our asymptotic theory covers situations when the observed processes associated with the SDEs are independently and identically distributed (iid), as well as when they are independently but not identically distributed (non-iid). In particular, we allow incorporation of available time-dependent covariate information into each SDE through a multiplicative factor of the drift function; we also permit different initial values and domains of observations for the SDEs. Our model selection problem thus encompasses selection of a set of appropriate time-dependent covariates from a set of available time-dependent covariates, besides selection of the part of the drift function free of covariates. For both iid and non-iid set-ups we establish almost sure exponential convergence of the Bayes factor. Furthermore, we demonstrate with simulation studies that even in non-asymptotic scenarios Bayes factor successfully captures the right set of covariates.

==> application.tex <==

\section{Simulation studies}
\label{sec:simulated_data}

\subsection{Covariate selection when $n=15$, $T=1$}
\label{subsec:N15T1}
We first demonstrate with simulation study the finite sample analogue of Bayes factor analysis
as $n\rightarrow\infty$ and $T$ is fixed. In this regard, we consider $n=15$ individuals, where the $i$-th one is modeled by
\begin{equation}
dX_i(t)=(\xi_1+\xi_2z_1(t)+\xi_3z_2(t)+\xi_4z_3(t))(\xi_5+\xi_6X_i(t))dt+\sigma_i dW_i(t),
\label{eq:sde2_appl}
\end{equation}
for $i=1,\cdots,15$. We fix our diffusion coefficients as $\sigma_{i+1}=\sigma_i +5$ for $i=1\cdots,14$ 
where $\sigma_1=10$. We consider the initial value $X(0)=0$ and the time interval $[0, T]$ with $T=1$. 
%Thus, compared to Section \ref{subsec:N1T5}, here there are more individuals but smaller time domain.
%As before, we consider $500$ discretized and equispaced time steps, using which we generated the data.

We obtain the true values of $\xi_i$; $i=1,\ldots,6$ as follows:
$\xi_{i}\stackrel{iid}{\sim} N(\mu_i,0.001^2)$, where 
$\mu_i\stackrel{iid}{\sim} N(0,1)$. This is not to be interpreted as the prior; this
is just a means to set the true vaues of the parameters of the data-generating model.
%Indeed, see for our purpose, we consider a multivariate normal prior for $\btheta$ with mean
%being the maximum likelihood estimator ($MLE$) and appropriate variance.
\\[2mm]
We assume that the time dependent covariates $z_i(t)$ satisfy the following $SDE$s 
\begin{align}
dz_1(t)=&(\tilde\theta_{1}+\tilde\theta_{2}z_1(t))dt+ dW_1(t)\notag\\
dz_2(t)=&\tilde\theta_{3}dt+ dW_2(t)\notag\\
dz_3(t)=&\tilde\theta_{4}z_3(t))dt+ dW_3(t),
\label{eq:covariate_appl}
\end{align}
where $W_i(\cdot)$; $i=1,2,3$, are independent Wiener processes, and 
$\tilde\theta_{i}\stackrel{iid}{\sim} N(0,0.01^2)$ for $i=1,\cdots,4$. 
%Here the diffusion coefficient $\sigma=1$. 

We obtain the covariates by first simulating $\tilde\theta_{i}\stackrel{iid}{\sim} N(0,0.01^2)$ for $i=1,\cdots,4$,
fixing the values, and then by simulating the covariates using the $SDE$s (\ref{eq:covariate_appl}) 
by discretizing the time interval $[0,5]$ into $500$ equispaced time points. 
In all our applications we have standardized the covariates over time so that they have zero means
and unit variances.

Once the covariates are thus obtained, we assume that the data are generated from the (true) model where all the covariates
are present. For the true values of the parameters, we simulated $(\xi_1,\ldots,\xi_6)$ from
the prior and treated the obtained values as the true set of parameters $\btheta_0$.
We then generated the data using (\ref{eq:sde2_appl}) by discretizing the time interval $[0,5]$ 
into $500$ equispaced time points.



As we have three covariates so we will have $2^3=8$ different models. Denoting
a model by the presence and absence of the respective covariates, it then is the case that 
$(1,1,1)$ is the true, data-generating model, while $(0,0,0)$, $(0,0,1)$, $(0,1,0)$, $(0,1,1)$, $(1,0,0)$,
$(1,0,1)$, and $(1,1,0)$ are the other $7$ possible models. 
%Now, we have to check values of the Bayes factor corresponding to $7$ different models. 

\subsubsection{Case 1: the true parameter set $\btheta_0$ is fixed}
\label{subsubsec:case1_appl}
{\bf Prior on $\btheta$}
\\[2mm]
%\label{subsubsec:case1_prior_BF}
For the prior $\pi$ on $\btheta$, we first 
obtain the maximum likelihood estimator ($MLE$) of $\btheta$ using simulated annealing
(see, for example, \ctn{Liu01}, \ctn{Robert04}), and
consider a normal prior where the mean is the $MLE$ of $\xi_i$ for $i=1,\ldots,6$ 
and the variance is $0.8^2\mathbb I_6$, $\mathbb I_6$ being the $6$-dimensional identity matrix. 
As will be seen, this results in consistent model selection using Bayes factor.
\\[2mm]
{\bf Form of the Bayes factor}
%\label{subsec:case1_bf}
\\[2mm]
In this case the related Bayes factor has the form
\begin{equation*}
I_n=\int \prod_{i=1}^n\frac {f_{i,\btheta_1}(X_i)}{f_{i,\btheta_0}(X_i)}\pi (d\btheta_1),
\label{eq:bf_T_appl}
\end{equation*}
where $\btheta_0=(\xi_{0,1},\xi_{0,2},\xi_{0,3},\xi_{0,4},\xi_{0,5},\xi_{0,6})$ is the true parameter set 
and $\btheta_1=(\xi_1,\xi_2,\xi_3,\xi_4,\xi_5,\xi_6)$ is the unknown set of parameters corresponding to 
any other model. 
%The prior distribution on the parameter set is denoted by $\pi$. The true likelihood is 
%$f_{\btheta_0,T}(X_{0,T})$. To check whether (\ref{eq:bf_appl}) holds we write $7$ 
%different wrong likelihoods in the place of $f_{\btheta_1,T}(X_{0,T})$ sequentially and obtain $7$ 
%different values of Bayes factor. 
%In this regard we use the $\btheta$ from a normal prior where 
%the mean is the $MLE$ of $\xi_i$ for $i=1,\cdots,6$ obtained by simulated annealing and variance is $0.8^2$. 
Table \ref{table:values} describes the results of our Bayes factor analyses. 
%where we denote the presence and absence of covariates by 1 and 0 respectively.
\begin{table}[h]
\centering
\caption{Bayes factor results}
\label{table:values}
\begin{tabular}{|c||c|}
\hline
Model & $\frac{1}{15}\log I_{15}$\\
\hline
$(0,0,0)$ & -3.25214\\ 
$(0,0,1)$ & -1.39209\\
$(0,1,0)$ & -3.31954\\
$(0,1,1)$ & -1.11729\\
$(1,0,0)$ & -3.40378\\
$(1,0,1)$ & -1.22529\\
$(1,1,0)$ & -3.46790\\
\hline
\end{tabular}
\end{table}
It is clear from the 7 values of the table that the correct model $(1,1,1)$ is always preferred.

\subsubsection{Case 2: the parameter set $\btheta_0$ is random and has the prior distribution $\pi$}
\label{subsubsec:case2_appl}
%{\bf Prior on $\btheta$}
%\\[2mm]
%\label{subsubsec:case2_prior_BF}
We consider the same form of the prior $\pi$ as in %Section \ref{subsubsec:case1_prior_BF}, 
Section \ref{subsubsec:case1_appl}, but with
variance $0.1^2\mathbb I_6$. The smaller variance compared to that in Case 1 attempts to somewhat 
compensate, in essence, for the lack of precise information about the true parameter values. 

In this case we calculate the marginal log-likelihood of the $8$ possible models as
$$\ell_i=\frac{1}{15}\log\int \prod_{i=1}^nf_{i,\btheta_1}(X_i)\pi (d\btheta_1);~i=1,\ldots,8,$$
with $\ell_8$ corresponding to the true model.
Table \ref{table:deltavalues} shows that $\ell_8$ 
is the highest. This clearly implies that 
the Bayes factor consistently selects the correct set of covariates even though the parameters of the true model are not fixed.
%As then 
%$$\frac{1}{5}E_{\btheta_0}\left[\left(\log\int f_{i,\btheta_1,5}(X_{0,5})\pi (d\btheta_1)\right)
%-\left(\log\int f_{\btheta_0,5}(X_{0,5})\pi (d\btheta_0)\right)\right]=\alpha_i-\alpha_0<0$$ for $i=1,\ldots,7$.
\begin{table}[h]
\centering
\caption{Values of $\frac{1}{15}\times$ marginal log-likelihoods}
\label{table:deltavalues}
\begin{tabular}{|c||c|}
\hline
Model & $\ell_i$\\
\hline
$(0,0,0)$ & 2.42430\\ 
$(0,0,1)$ & 4.29608\\
$(0,1,0)$ & 1.75213\\
$(0,1,1)$ & 4.84717\\
$(1,0,0)$ & 1.56242\\
$(1,0,1)$ & 4.92628\\
$(1,1,0)$ & 0.47111\\
$(1,1,1)$ & 5.84665 ($\mbox{true model}$)\\
\hline
\end{tabular}
\end{table}

\subsection{Covariate selection when $n=1$, $T=5$}
\label{subsec:N1T5}

We now assume the same set-up as Section \ref{subsec:N15T1}, but set $n=1$, $T=5$, and 
for the diffusion coefficient, set $\sigma_1=\sigma=20$.
As per our theory, for a single individual, the Bayes factor is not consistent for increasing time domain.
However, we have shown that 
\begin{equation*}
\frac{1}{T}E_{\btheta_0}(\log I_T)\rightarrow -\delta
\label{eq:bf_appl}
\end{equation*}
as $T\rightarrow \infty$. Thus, the Bayes factor is consistent with respect to the expectation. 
Our simulation results show that this holds even for the time domain $[0,5]$,
where we approximate the expectation with the average of %$500$ 
$1000$ realizations of $I_T$
associated with as many simulated data sets. %case we have simulated the data 500 times to verify the result (\ref{eq:bf_appl}). 


\subsubsection{Case 1: the true parameter set $\btheta_0$ is fixed}
\label{subsubsec:case1_appl2}
{\bf Prior on $\btheta$}
\\[2mm]
As Section \ref{subsubsec:case1_appl}, 
we obtain the maximum likelihood estimator ($MLE$) of $\btheta$ using simulated annealing
and consider a normal prior with the $MLE$ as the mean and variance $0.8^2\mathbb I_6$.
\\[2mm]
{\bf Form of the Bayes factor}
%\label{subsec:case1_bf}
\\[2mm]
In this case the related Bayes factor has the form
\begin{equation}
I_T=\int \frac {f_{\btheta_1,T}(X_{0,T})}{f_{\btheta_0,T}(X_{0,T})}\pi (d\btheta_1),
\label{eq:bf_T_appl2}
\end{equation}
where $\btheta_0=(\xi_{0,1},\xi_{0,2},\xi_{0,3},\xi_{0,4},\xi_{0,5},\xi_{0,6})$ is the true parameter set 
and $\btheta_1=(\xi_1,\xi_2,\xi_3,\xi_4,\xi_5,\xi_6)$ is the unknown set of parameters corresponding to 
any other model. 
%The prior distribution on the parameter set is denoted by $\pi$. The true likelihood is 
%$f_{\btheta_0,T}(X_{0,T})$. To check whether (\ref{eq:bf_appl}) holds we write $7$ 
%different wrong likelihoods in the place of $f_{\btheta_1,T}(X_{0,T})$ sequentially and obtain $7$ 
%different values of Bayes factor. 
%In this regard we use the $\btheta$ from a normal prior where 
%the mean is the $MLE$ of $\xi_i$ for $i=1,\cdots,6$ obtained by simulated annealing and variance is $0.8^2$. 
Table \ref{table:values2} describes the results of our Bayes factor analyses. 
%where we denote the presence and absence of covariates by 1 and 0 respectively.
\begin{table}[h]
\centering
\caption{Bayes factor results}
\label{table:values2}
\begin{tabular}{|c||c|}
\hline
Model & Averaged $\frac{1}{5}\log I_5$\\
\hline
$(0,0,0)$ & -2.5756029\\ 
$(0,0,1)$ & -0.913546\\
$(0,1,1)$ & -0.5454860\\
$(0,1,0)$ & -0.763952\\
$(1,0,0)$ & -2.5774163\\
$(1,0,1)$ & -0.9312218\\
$(1,1,0)$ & -0.7628154\\
\hline
\end{tabular}
\end{table}
It is clear from the 7 values of the table that the correct model $(1,1,1)$ is always preferred.

\subsubsection{Case 2: the parameter set $\btheta_0$ is random and has the prior distribution $\pi$}
\label{subsubsec:case2_appl2}
%{\bf Prior on $\btheta$}
%\\[2mm]
%\label{subsubsec:case2_prior_BF}
As before, we consider the same form of the prior as in Section \ref{subsubsec:case1_appl2},
but with variance $0.1^2\mathbb I_6$. 
In this case we calculate marginal likelihood of the 8 possible models, and approximate
$$\frac{1}{5}E_{\btheta_0}\left(\log\int f_{i,\btheta_1,5}(X_{0,5})\pi (d\btheta_1)\right)$$ for $i=1,\ldots,8$ by 
averaging over $1000$ replications of the data obtained from the true model. 
Denoting its values by $\ell_i$,  Table \ref{table:deltavalues2} shows that $\ell_8$ 
is the highest, implying consistency of the averaged Bayes factor.
\begin{table}[h]
\centering
\caption{Averages of $\frac{1}{5}\times$ marginal log-likelihood}
\label{table:deltavalues2}
\begin{tabular}{|c||c|}
\hline
Model & $\ell_i$\\
\hline
$(0,0,0)$ & -1.21923\\ 
$(0,0,1)$ & -0.21428\\
$(0,1,0)$ & 1.47992\\
$(0,1,1)$ & 2.102966\\
$(1,0,0)$ & -1.222362\\
$(1,0,1)$ & -0.21898\\
$(1,1,0)$ & 1.459921\\
$(1,1,1)$ & 2.121237 ($\mbox{true model}$)\\
\hline
\end{tabular}
\end{table}

\begin{comment}
\subsubsection{Posterior predictive inference for the chosen model}
\label{subsubsec:conv_parameter}

We now evaluate the performance of the selected model by means of posterior predictive inference. Specifically,
we attempt to predict the last $50$ observations, given the first $450$. 
For this, we first sample from the posterior of $\btheta_1=(\xi_1,\xi_2,\xi_3,\xi_4,\xi_5,\xi_6)$
given the first $450$ observations, and given each realized value of $\btheta_1$ from this posterior,
we obtain the discretized time series for the last $50$ observations, after sampling the Wiener process
for the last $50$ time points conditional on the Wiener process for the first $450$ time points. 
For posterior predictive inference we assume the following prior: for $i=1,\ldots,6$, 
$\xi_i\stackrel{iid}{\sim}N(0,0.0006^2)$.

We sampled from the posterior of $\btheta_1$ using Transformation based Markov Chain Monte Carlo (TMCMC)
introduced by \ctn{SS2012}, considering the additive transformation in particular. 
The importance of TMCMC is that it updates high-dimensional parameters in a single
block using suitable deterministic transformations of arbitrary low-dimensional/one-dimensional
random variables defined on some relevant support. So this method drastically reduces dimension, which,
in turn, significantly reduces computational burden and improves acceptance rate. 

In a nutshell, first we fix an initial (old) value $\xi_{i,old}$; $i=1,\ldots,6$, which we simulate from the prior. 
At each iteration of additive TMCMC we then propose an update of the form
$\xi_{i,new}=\xi_{i,old}+b_i a |\epsilon|$ for $i=1,\cdots,6$, , where 
$b_i$ such that $b_i=\pm 1$ with probability $1/2$, $\epsilon \sim N(0,1)$ and $a=0.01$ is a tuning parameter.
Let $\ell_{new}-\ell_{old}$ denote the difference between the log-likelihood evaluated at the
new and old values of the parameters. If $\log u\leq \ell_{new}-\ell_{old}$,
we update the old values of the parameters, otherwise, we retain 
the old values.
We have thus simulated $150000$ TMCMC realizations from the posterior. 

We found that the TMCMC convergence of the parameters are good under considered prior distribution. 
Here we have shown the TMCMC convergence of the parameters under the prior $N(0,0.006^2)$ by Figure \ref{fig:posteriors}.

\begin{figure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi1.pdf}
\label{fig:sfig1}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi2.pdf}
\label{fig:sfig2}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi3.pdf}
\label{fig:sfig3}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi4.pdf}
\label{fig:sfig4}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi5.pdf}
\label{fig:sfig5}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/xi6.pdf}
\label{fig:sfig6}
\end{subfigure}
\caption{TMCMC convergence of the posterior distribution of the parameters}
\label{fig:posteriors}
\end{figure}

\subsubsection{Posterior Predictives}
\label{subsubsec:pp}

Conditioning on the Brownian motions for the first 450 time poins we obtain the Brownian motion for the last 50 time points which will be useful for the evaluation of posterior predictives of the last 50 data points. By thinning from 150000 posterior values of the parameter set we have chosen 1000 values. Corresponding to 1000 values of the parameter set we will have 1000 posterior predictives which we denote by $Yp_j$  for $j=1,\cdots,1000$. 

From (\ctn{Sabya11}) we get the idea of obtaining the modes and any desired highest posterior density credible regions associated with the posterior distribution. With the help of that idea we define posterior mode of $Yp_j$  for $j=1,2,\cdots,N$ as
$$P(\{Yp_j:d(Yp^*,Yp_j)< \epsilon\})=\underset{Yp_i; 1\leq i\leq N}{\sup} P(\{Yp_j:d(Yp_i,Yp_j)< \epsilon\})$$
where the metric $d$ is chosen as supnorm metric and $N=1000$.
 For $N=1000, Yp^*$ is caculated emperically by
$$Yp^*=\underset{1\leq i\leq N }{\arg \max}\frac{1}{N}\#\{Yp_j; 1\leq j\leq N:d(Yp_i,Yp_j)< \epsilon\}.$$
 Given $Yp^*,$ $95\%$ posterior density credible region is obtained as the set 

$\{Yp_j; 1\leq j\leq N:d(Yp^*,Yp_j)< \epsilon^*\}$ where $\epsilon^*$ is such that
$$\frac{1}{N}\#\{Yp_j; 1\leq j\leq N:d(Yp^*,Yp_j)< \epsilon^*\}\approx 0.95$$

We also find the posterior predictive from which the distance of the true data is minimum (call it as minimum posterior predictive) and calculate $95\%$ posterior density credible region around it as the same way as mentioned in the case of posterior mode. 

Now, to conclude which posterior predictive we will chose, for that we note the distance of posterior mode from true data (denoted by PMD) and the radius of $95\%$ posterior density credible region around it (denoted by PMDR). Besides, we also note the minimum distance of posterior predictive from the true data (denoted by MD) and the radius of $95\%$ posterior density credible region around that particular posterior predictive (denoted by MDR). Now by comparing the sum of PMD and PMDR (denoted by $T_{PM}$) and the sum of MD and MDR (denoted by $T_{M}$) whichever is minimum we consider that particular posterior predictive as our required posterior predictive. In our case we find $T_M$ is minimum. The figure \ref{fig:figpp} shows the posterior predictives along with true data in which by "minimum" we mean that posterior predictive from which the distance of the true data is minimum.

\begin{figure}
\centering
\includegraphics[height=10cm,width=9cm]{Application/data1time5.pdf}
\caption{Posterior Predictive for N=1, T=5}
\label{fig:figpp}
\end{figure}

\end{comment}

\begin{comment}
\subsection{Comparison between different models for more than one individual}
\label{subsec:N15T1}

We now consider $15$ individuals, where the $i$-th one is modeled by
\begin{equation}
dX_i(t)=(\xi_1+\xi_2z_1(t)+\xi_3z_2(t)+\xi_4z_3(t))(\xi_5+\xi_6X_i(t))dt+\sigma_i dW_i(t),
\label{eq:sde2_appl}
\end{equation}
for $i=1,\cdots,15$. We fix our diffusion coefficients as $\sigma_{i+1}=\sigma_i +5$ for $i=1\cdots,14$ 
where $\sigma_1=10$. We consider the initial value $X(0)=0$ and the time interval $[0, T]$ with $T=1$. 
Thus, compared to Section \ref{subsec:N1T5}, here there are more individuals but smaller time domain.
As before, we consider $500$ discretized and equispaced time steps, using which we generated the data.
%We break the time domain in 500 time points i.e we break the time interval with the step size 0.002. 

Here our covariates and the true parameter set $\btheta_0=(\xi_{0,1,}\xi_{0,2},\xi_{0,3},\xi_{0,4},\xi_{0,5},\xi_{0,6})$  
are simulated in a similar way as described in Section  \ref{subsec:N1T5}. 

For each of the $15$ individuals, we selected the covariate combination randomly. Thus, 
Also we compare this combination with other $100$ different covariate combinations for these $15$ 
individuals to check whether Bayes Factor can select the correct combination.

In this case our related Bayes Factor corresponding to j-th covariate combination
\begin{align}
I_N^j&=\int  R_N^j(\btheta_1)\pi(d\btheta_1),
\label{eq:I_n_appl}
\end{align}
 where
\[
R_N^j(\btheta_1)=\prod_{i=1}^N\frac{f^j_{i,\btheta_1}(X_i)}{f_{i,\btheta_0}(X_i)}.
\]
for $j=1,\cdots,100$ where $\btheta_0$ is the true parameter set. Note  that in our set-up, N=15.

Firstly, by simulated annealing we obtain the MLE of the parameter set. Then we calculate the Bayes factor by taking the normal prior with mean as the respective MLEs and variance 1. In all the cases corresponding to 100 covariate combinations we obtain
$\frac{1}{N}\log I^j_{N}$ i.e. $$\frac{1}{15}\log I^j_{15}=-\delta_j$$ for $j=1,\cdots,100$. This shows that Bayes Factor indicates the correct covariate combination. As in section 
\ref{subsec:bf_appl} we also consider the case when the true covariate combination is unknown to us. We denote the joint likelihood corresponding to j-th covariate combination by $\prod_{i=1}^{15}f^j_{i,\btheta_1}(X_{i})$ and that corresponding to true covariate combination by $\prod_{i=1}^{15}f_{i,\btheta_0}(X_{i})$.  With respect to the normal prior with mean as obtained from simulated annealing and variance $0.1^2$  we find

$$\frac{1}{15}\left[\left(\log\int \prod_{i=1}^{15}f^j_{i,\btheta_1}(X_{i})\pi (d\btheta_1)\right)-\left(\log\int \prod_{i=1}^{15}f_{i,\btheta_0}(X_{i})\pi (d\btheta_0)\right)\right]=\alpha_j-\alpha_0<0$$ for $j=1,\cdots,100,$ as maximum value of $\alpha_j$  is -0.118787 among 100 values of $\alpha_j$ and $\alpha_0=1.31028$. This result indicates that though the correct covariate combination is unknown to us we are able to find that combination.

 After getting the true covariate combination for 15 individuals we want to predict the last 50 time points for each individual by conditioning on first 450 time points as mentioned in section \ref{subsubsec:pp}. The process of obtaining posterior predictives is same as described in section \ref{subsubsec:pp}. Here also after obtaining the posterior mode and the posterior predictive from which the distance of true data is minimum we calculate $T_{PM}$ and $T_M$.  In the figure \ref{fig:pp2} in case of 1st and 6th data we find $T_M$ is minimum. For the 7th data the posterior mode and the posterior predictive from which the distance of the true data is minimum (which is denoted in other two figures by "minimum") coincide.


\begin{figure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/data15time11st.pdf}
\label{fig:sfig8}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/data15time16th.pdf}
\label{fig:sfig9}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/data15time17th.pdf}
\label{fig:sfig10}
\end{subfigure}
\caption{Posterior Predictives of 3 Data}
\label{fig:pp2}
\end{figure}

\end{comment}

\subsection{Bayes factor analysis for $n=15$ and $T=5$}
\label{subsec:N15T5}

In this case we allow our parameter and the covariate sets to vary from individual to individual. 
We consider $15$ individuals modeled by
\begin{equation}
dX_i(t)=(\xi_1^i+\xi_2^iz_1(t)+\xi_3^iz_2(t)+\xi_4^iz_3(t))(\xi_5^i+\xi_6^iX_i(t))dt+\sigma_i dW_i(t)
\label{eq:sde3_appl3}
\end{equation}
for $i=1,\cdots,15$. We fix our diffusion coefficients as $\sigma_{i+1}=\sigma_i +5$ for $i=1\cdots,14$ 
where $\sigma_1=10$. We consider the initial value $X(0)=0$ and the interval $[0, T]$, with $T=5$. 
As before, we generated the observed data after discretizing the time interval into $500$ equispaced time points. 
%We break the time domain in 500 time points i.e we break the time interval with the step size 0.01. 
Here our covariates and the parameter set 
$\btheta_0^i=(\xi_{0,1}^i,\xi_{0,2}^i,\xi_{0,3}^i,\xi_{0,4}^i,\xi_{0,5}^i,\xi_{0,6}^i)$; $i=1,\ldots,15$, 
are simulated in a similar way as mentioned in Section \ref{subsec:N1T5}.

For each of the $15$ individuals, the true set of covariate combination is randomly selected. 
Thus, for a given model, there are $15$ sets of covariate combinations to be compared with other models
consisting of $15$ different sets of covariate combinations.
To decrease computational burden we compare the true model with $100$ other models consisting of 
different sets of covariate combinations. 

The Bayes factor corresponding to the $j$-th covariate combination is given by
\begin{equation}
I_{nT}^j=\prod_{i=1}^n\int \frac{f^j_{i,\btheta^{(i)}_1}(X_{i,0,T})}
{f_{i,\btheta^{(i)}_0}(X_{i,0,T})}\pi\left(\btheta^{(i)}_{1}\right)d\btheta^{(i)}_{1}
\label{eq:I_iT_appl}
\end{equation}
for $j=1,\cdots,1000$, where $n=15$, $T=5$ and $\btheta_0^{(i)}$ is the true parameter set corresponding to 
the $i$-th individual.

We obtain the $MLE$ of the $15$ parameter sets by simulated annealing. Then we calculate the Bayes factor 
with the prior such that the parameter components are independent normal with means as the respective $MLE$s and variances $1$. 
In all the cases corresponding to $100$ covariate combinations we obtain 
$\frac{1}{nT}\log I^j_{nT}<0$ for $j=1,\cdots,100$. 
Thus, Bayes factor indicated the correct covariate combination in all the cases considered. 
%As in section \ref{subsec:bf_appl} 
We also considered the case when a normal prior is considered for the parameters of the true model. 
In this case with respect to the component-wise independent normal prior with individual mean as obtained 
from simulated annealing and component-wise variance $0.1^2$, we obtain 
\begin{equation}
\frac{1}{15\times 5}\left[\log\left(\prod_{i=1}^{15}\int f^j_{i,\btheta_1^{(i)}}(X_{i,0,T})
\pi(\btheta^{(i)}_1)d\btheta_1^{(i)}\right)-\log\left(\prod_{i=1}^{15}\int f_{i,\btheta_0^{(i)}}(X_{i,0,T})
\pi(\btheta^{(i)}_0)d\btheta_0^{(i)}\right)\right]<0, %=\ell_j-\ell_0<0
\label{eq:INT_appl}
\end{equation}
for $j=1,\cdots,100$. Indeed, it turned out that 
$\frac{1}{15\times 5}\log\left(\prod_{i=1}^{15}\int f_{i,\btheta_0^{(i)}}(X_{i,0,T})
\pi(\btheta^{(i)}_0)d\btheta_0^{(i)}\right)=0.4865$ 
and the maximum of 
$\frac{1}{15\times 5}\log\left(\prod_{i=1}^{15}\int f_{i,\btheta^{(i)}}(X_{i,0,T})
\pi(\btheta^{(i)})d\btheta^{(i)}\right)$ is $0.4127$.
In other words, the Bayes factor consistently selects the correct model even in this situation.


\section{Company-wise data from national stock exchange}
\label{sec:truedata} 

To deal with real data we collect the stock market data 
($467$ observations during the time range August $5$, 2013, to June $30$, 2015) 
for $15$ companies which is available on 
{\it www.nseindia.com}. 
Each company-wise data is modeled by various availabe standard financial $SDE$ 
models with the available ``fitsde" package in $R$. After obtaining the BIC (Bayesian Information Criterion) 
for each company corresponding to each available financial model, we find that the minimum value of BIC corresponds to 
the $CKLS$ model, given, for process $X(t)$, by
$$dX(t)=(\theta_1+\theta_2X(t))dt+\theta_3X(t)^{\theta_4}dW(t).$$
As per our theory we treat the diffusion coefficient as a fixed quantity. 
So, after obtaining the estimated value of the coefficients by the ``fitsde" function, 
we fix the values of $\theta_3$ and $\theta_4$, so that the diffusion coefficient becomes fixed.
We let $\theta_3=A$, $\theta_4=B$.


In this $CKLS$ model, we now wish to include time varying covariates. 
In our work we consider the ``close price" of each company. The stock market data is assumed to 
be dependent on IIP general index, bank interest rate, US dollar exchange rate and on various other quantities. 
But we assume only these three quantities as possibly the most important time dependent covariates. 

Briefly, IIP, that is, index of industrial production, is a measurement which represents 
the status of production in the industrial sector for a given period of time compared to a reference period of time. 
It is one of the best statistical data, which helps us measure the level of industrial activity in Indian economy. 
Its importance lies in the fact that low industrial production  will result in lower corporate sales and profits, 
which will directly affect stock prices. So a direct impact of weak IIP data is a sudden fall in stock prices. 

As the IIP data is purely industrial data, banking sector is not included in it. So, 
we also consider the bank interest rate as another covariate. Note that, higher the bank interest rate, 
fixed deposits become more attractive and one will preferably deposit money in bank rather than invest in stock market. 
Besides, companies with a high amount of loans in their balance sheets would be affected very seriously. 
Interest cost on existing debt would go up affecting their EPS (Earning per Share) and ultimately the stock prices. 
But during low interest rate these companies would stand to gain. Banking sector is likely to benefit most due 
to high interest rates. The Net Interest Margins (it is the difference between the interest they 
earn on the money they lend and the interest they pay to the depositors) for banks is likely to 
increase leading to growth in profits and the stock prices. Hence, it is clear that, the interest rates 
and stock markets are inversely related. As the interest rates go up, stock market 
activities tend to come down. 

Finally, exchange rates directly affect the realized return on 
an investment portfolio with overseas holdings. If one own stock in a foreign company and the 
local currency goes up, the value of the investment also goes up. 
Foreign investment is also related very much to US dollar exchange rate.

Hence, we collect the values of the aforementioned time varying covariates 
during the time range August $5$, 2013, to June $30$, 2015. 
We denote these three quantities by $c_1,c_2,c_3$ respectively. Now, our considered $SDE$ models
for national stock exchange data associated with the $15$ companies are the
following:
\begin{equation}
dX_i(t)=(\theta_1^i+\theta_2^ic_1(t)+\theta_3^ic_2(t)+\theta_4^ic_3(t))(\theta_5^i+\theta_6^iX_i(t))dt+A^iX_i(t)^{B^i}dW_i(t),
\label{eq:sde4_appl}
\end{equation}
for $i=1,\cdots,15$. 
%It is important to mention that we are able to find out $467$ 
%data points which implies our data is observed in [0, 467] i.e. T=467.

\subsection{Selection of covariates by Bayes factor}
\label{subsec:covariate_bf}

Among the considered three time varying covariates we now select the best set of covariate combinations
for the $15$ companies from among $100$ such sets through Bayes factor, 
computing the log-marginal-likelihoods with respect to the normal prior
on the parameter set, assuming {\it a priori} independence of the parameter components 
with individual means being the corresponding $MLE$ (based on simulated annealing)
and unit variances.
Table \ref{table:companies} provides the sets of covariates for the $15$ companies obtained
by our Bayes factor analysis. Also observe that each of the three covariates occurs about $50\%$ times
among the companies, demonstrating that overall impact of these on national stock exchange is
undeniable.
\begin{table}[h]
\centering
\caption{Company-wise covariates obtained by Bayes factor analysis}
\label{table:companies}
\begin{tabular}{|c||c|}
\hline
Company & Covariates\\
\hline
$1$ & Bank rate\\ 
$2$ & US dollar exchange rate\\
$3$ & None\\
$4$ & None\\
$5$ & Bank rate and US dollar exchange rate\\
$6$ & Bank rate and US dollar exchange rate\\
$7$ & IIP general index and US dollar exchange rate\\
$8$ & Bank rate\\
$9$ & IIP general index and Bank rate\\
$10$ & IIP general index\\
$11$ & IIP general index, Bank rate and US dollar exchange rate\\
$12$ & IIP general index and Bank rate\\
$13$ & US dollar exchange rate\\
$14$ & IIP general index, Bank rate and US dollar exchange rate\\
$15$ & IIP general index\\
\hline
\end{tabular}
\end{table}


%For that we have done simulated annealing for the 15 parameter sets. 
%Considering $100$ different covariate combinations for 15 companies we find a certain combination appropriate for 15 companies by Bayes Factor. Note that, our set up is similar to the setup considered in section \ref{subsec:N15T5} except T=467. Hence, according to equation \ref{eq:INT_appl}
%for $j=1,\cdots,100$ the highest value of $\alpha_j$ corresponds to the appropriate combination among 100 combinations. We have shown here three companies among which 2nd company is dependent on IIP and Bank rate. IIP and USD exchange rate are important for 13th company and for 15th company Bank rate and USD exchange rate is important.

\begin{comment}
Here also after obtaining posterior distribution of parameters by TMCMC method we find the posterior predictives of last 47 time point by conditioning on first 420 time points exactly in the same way as described in section \ref{subsec:N1T5} . Figure \ref{fig:pp4} describes the posterior predictives of three companies. In all the cases we calculate $T_{PM}$ and $T_M$ and find that in each case $T_M$ is minimum. Hence ``minimum" will be our required posterior predictives.

\begin{figure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/C14.pdf}
\label{fig:sfig8_3}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/C50.pdf}
\label{fig:sfig9_3}
\end{subfigure}
\begin{subfigure}
\centering
\includegraphics[height=6cm,width=5cm]{Application/C63.pdf}
\label{fig:sfig10_3}
\end{subfigure}
\caption{Posterior Predictives of 3 Company}
\label{fig:pp4}
\end{figure}

\end{comment}

